(Anti-)De Sitter null strings and Carroll-Weyl symmetry

We construct a $dS_d$ null string in a novel way by lifting the standard tensionless string to $R^{1,d}$. Gauging worldsheet scale symmetry introduces terms in the action breaking translation invariance, but preserving the $dS_d$ symmetry $SO(1,d)$. Choosing a De Sitter symmetric gauge fixing of the scale symmetry yields a $d$ dimensional theory which we show has all the expected properties of $dS_d$ tensionless strings. The action happens to be the intriguing Carrol-Weyl symmetric string action in $R^{1,d}$, now with a clear target space interpretation in $d$ dimensions. That it does not, as recently claimed, represent a ($d+1$)-dimensional string in flat ($d+1$)-dimensional Minkowski space settles an apparent issue with the Carrol-Weyl string model. Furthermore, while there are clear obstacles for similar formulations of tensile strings in (A)dS backgrounds, our new insights are easily modified to the formulation of Anti-De Sitter tensionless strings. That our construction generates a curved geometry purely algebraically may have even wider applications.

==> macros.tex <==
% IMPORTS
\usepackage{physics}
\usepackage{tensor}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage[colorlinks=true]{hyperref}
\usepackage{xcolor}
\usepackage{cancel}
\usepackage{ytableau}
\usepackage{marginnote}

%TITLES AND SECTIONS
\usepackage{titlesec}
\makeatletter
\g@addto@macro\bfseries{\boldmath}
\makeatother

\ytableausetup{boxsize=0.3em,centertableaux}

% MISC
\usepackage{framed}
\usepackage[most]{tcolorbox}
\usepackage{xcolor}
\colorlet{shadecolor}{gray!10}

% DEFINITIONS
\newcommand{\cov}{\nabla}

\newcommand{\nn}{\nonumber}
\newcommand{\al}{\alpha} 
\newcommand{\be}{\beta}
\newcommand{\ga}{\gamma}
\newcommand{\Ga}{\Gamma}
\newcommand{\de}{\delta}
\newcommand{\ka}{\kappa}
\newcommand{\vp}{\varphi}
\newcommand{\La}{\Lambda}
\newcommand{\la}{\lambda}
\newcommand{\Om}{\Omega}




\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}

